Online Stochastic Matching with Edge Arrivals

Online bipartite matching with edge arrivals remained a major open question for a long time until a recent negative result by [Gamlath et al. FOCS 2019], who showed that no online policy is better than the straightforward greedy algorithm, i.e., no online algorithm has a worst-case competitive ratio better than $0.5$. In this work, we consider the bipartite matching problem with edge arrivals in a natural stochastic framework, i.e., Bayesian setting where each edge of the graph is independently realized according to a known probability distribution. We focus on a natural class of prune & greedy online policies motivated by practical considerations from a multitude of online matching platforms. Any prune & greedy algorithm consists of two stages: first, it decreases the probabilities of some edges in the stochastic instance and then runs greedy algorithm on the pruned graph. We propose prune & greedy algorithms that are $0.552$-competitive on the instances that can be pruned to a $2$-regular stochastic bipartite graph, and $0.503$-competitive on arbitrary bipartite graphs. The algorithms and our analysis significantly deviate from the prior work. We first obtain analytically manageable lower bound on the size of the matching, which leads to a non linear optimization problem. We further reduce this problem to a continuous optimization with a constant number of parameters that can be solved using standard software tools.

==> analysis.tex <==
\begin{itemize}
	\item $\exists e, \exists (uv)$: $e$ is realized, at least one edge of $E_{uv}$ is realized;
	\item $y_e, y_{uv}$: the corresponding probabilities;
	\item $Q_v(u), Q_v(e)$: $v$ has no realized edge before $(vu),e$;
	\item $q_v(u), q_v(e)$: probability;
\end{itemize}

In this section, we establish a general lower bound on the performance of the greedy algorithm with respect to the worst-case arrival order.
Let $G$ be a stochastic graph in which each edge $e$ exists independently with probability $y_e$. Let $x_e = \epsilon$ for all edges in $G$. We should think of in the regular graph case, $y_e = c \epsilon$ and in the general graph case, $y_e = \min (p_e, c \epsilon)$. However, to derive the lower bound, we only use the fact $y_e \le c\epsilon$ that holds for both cases.

Observe that the expected performance of greedy equals the expected number of vertices being matched in $L$ according to the bipartiteness of the graph. We start by studying the matching probability of each vertex in $L$ and then carefully divide the gain into its incident edges. Note that we shall break the symmetry of $L, R$ in our analysis. 
Define the following two types of contributions of each edge $e \in E_{vu}$, where $v\in L$ and $u \in R$:
\begin{align*}
& \rone(e) \eqdef x_{e} \cdot \left( 1 - \exp \left( - \frac{q_u(e)\cdot y_e}{x_e} \right) \right); \\
\text{and } & \rtwo(e) \eqdef y_{e} \cdot \left( \Pr{\overline{M_{u}}(e)} - \Pr{Q_{u}(e)}  \right).
\end{align*}

\begin{lemma}
	\label{lem:greedy_analysis}
\begin{equation}
\greedy \ge \sum_{v \in L} \sum_{e \in E_v} \left( \rone(e) + e^{-c-ce^{-c}} \cdot \rtwo(e) \right) = \sum_{u \in R} \sum_{e \in E_u} \left( \rone(e) + e^{-c-ce^{-c}} \cdot \rtwo(e) \right).
\end{equation}	
\end{lemma}

Noticeably, the bound holds only on average but not edge-wise, i.e. $\rone(e) + e^{-c-ce^{-c}} \cdot \rtwo(e)$ might not be a lower bound of the probability that $e$ is matched for every $e$. 
Observe that the probability events involved in $\rone(e)$ and $\rtwo(e)$ are all local events of $u \in R$.
By dividing the gain into edges, it allows us to change the summation over vertices in $R$ and study the incident edges to each vertex in $R$ locally.

The proof of the lemma is technical, while the two parts of gains $\rone(e),\rtwo(e)$ admit meaningful interpretation. We sketch our plan before we provide the formal proof.
\begin{enumerate}
\item We first prove that in the worst-case arrival order, all parallel edges arrive consecutively. Thus, we may consider all parallel edges in $E_{vu}$ as a single batched-edge $(vu)$.
\item We analyze the probability that $v$ is matched. We say $u$ is a witness of $v$ if edge $(vu)$ exists and upon $(vu)$'s arrival, $u$ remains unmatched. We prove that $v$ must be matched if it admits at least one witness. If the events of being a witness of $v$ are independent, the bound can be written explicitly. Unfortunately, this might not be true in general. To proceed, we relax the event $\overline{M_u}(v)$ to be $Q_{u}(v)$ so that $Q_{u}(v)$ are independent across different $u$'s. This part would then corresponds to $\rone$. Moreover, we are able to retrieve some extra gain by considering the event that $(vu)$ is the only realized edge of $v$, that corresponds to $\rtwo$.
\item The final step is a subdivision lemma that is mainly technical. The previous step holds only for batched-edges. Informally, we show that the worst case is achieved when every batched-edge only consists of one small edge.
\end{enumerate}

\subsection{Proof of Lemma~\ref{lem:greedy_analysis}}
%Note that the greedy algorithm is non-adaptive to the arrival order of the edges. 
Let $\greedy_\sigma$ be the expected performance of the greedy algorithm with respect to arrival order $\sigma$ and $\greedy_\sigma(F)$ be the performance of the greedy algorithm when $F$ is the set of realized edges.

Our first lemma shows that the worst-case order $\sigma$ of edge arrivals would put all parallel edges into consecutive batches.

\begin{lemma}
For any arrival order $\sigma$,	for any two parallel edges $e_1=e_2=(uv)$ that $e_1$ arrives earlier than $e_2$, let $\sigma_1$ be the arrival order that postpones $e_1$ to arrive right before $e_2$ and $\sigma_2$ be the arrival order that expediting $e_2$ to arrive right after $e_1$.
Then $\greedy_\sigma \ge \min \left( \greedy_{\sigma_1}, \greedy_{\sigma_2} \right)$.
\end{lemma}

\begin{proof}
For arrival order $\sigma$, the performance performance of greedy would not depend on the existence of $e_2$ if $e_1$ exists, since it either accepts $e_1$, or at least one of $u,v$ is already matched before $e_1$'s arrival.
Let $A_1 = \Ex[F]{\greedy_\sigma(F) | \exists e_1}$, $A_2 = \Ex[F]{\greedy_\sigma(F) | \nexists e_1, \exists e_2}$ and $A_3 = \Ex[F]{\greedy_\sigma(F) | \nexists e_1,e_2}$. Then
\[
\greedy_\sigma = y_{e_1} A_1 + (1-y_{e_1})y_{e_2} A_2 + (1-y_{e_1})(1-y_{e_2}) A_3.
\]
Moreover, we have that
\begin{align*}
\greedy_{\sigma_1} = & (y_{e_1}+y_{e_2}-y_{e_1}y_{e_2}) \Ex[F]{\greedy_{\sigma_1}(F) | \exists e_1 \mbox{ or } e_2} + (1-y_{e_1})(1-y_{e_2}) \Ex[F]{\greedy_{\sigma_1}(F) | \nexists e_1,e_2} \\
= & (y_{e_1}+y_{e_2}-y_{e_1}y_{e_2}) A_1 + (1-y_{e_1})(1-y_{e_2}) A_3,
\end{align*}
and similarly,
\begin{align*}
\greedy_{\sigma_2} = & (y_{e_1}+y_{e_2}-y_{e_1}y_{e_2}) \Ex[F]{\greedy_{\sigma_2}(F) | \exists e_1 \mbox{ or } e_2} + (1-y_{e_1})(1-y_{e_2}) \Ex{\greedy_{\sigma_2}(F) | \nexists e_1,e_2} \\
= & (y_{e_1}+y_{e_2}-y_{e_1}y_{e_2}) A_2 + (1-y_{e_1})(1-y_{e_2}) A_3.
\end{align*}
To conclude the proof, observe that $\greedy_\sigma$ is a convex combination of $\greedy_{\sigma_1}$ and $\greedy_{\sigma_2}$.
\end{proof}

From now on, we assume edges in $E_{uv}$ arrive consecutively for any pair of vertices $u,v$. For the ease of presentation, we also think of the edges in $E_{uv}$ as a single batched-edge and use $(uv)$ to denote it. We use $\exists (uv)$ to denote the event that this batched-edge is realized, i.e. at least one edge of $E_{uv}$ is realized, and use $y_{uv}$ to denote the probability of this event, i.e. $y_{uv} = 1 - \prod_{e\in E_{uv}}(1-y_e)$.

Let $v$ be any fixed vertex in $L$ and $u_1,u_2,\cdots u_n$ be the neighbors of $v$ in $R$ enumerated according to the arrival order of the edges $(vu_i)$.

\begin{lemma}
	\label{lem:prob_v_match}
\begin{equation}
\Pr{M_v}\ge\Pr{\bigcup_{i=1}^n \left( Q_{u_i}(v)\cap \exists(vu_i) \right)}+
\sum_{i=1}^{n} \Pr{\overline{M_{u_i}}(v) \backslash Q_{u_i}(v) \cap \exists(vu_i) \cap_{j \ne i} \nexists(vu_j)}
\label{eq:estimate_matching}
\end{equation}
\end{lemma}

\begin{proof}
First of all, we prove that if $u_i$ is unmatched before $(vu_i)$ and the edge $(vu_i)$ is realized, then $v$ is matched, i.e.
\[
\overline{M_{u_i}}(v)\cap \exists(vu_i) \in M_v, \forall i \in [n].
\]
Consider the moment when edge $(vu_i)$ arrives, since $u_i$ remains unmatched, either $v$ is matched before $(vu_i)$, or $v$ will be matched to $u_i$ at this point. Therefore,
\[
\Pr{M_v} \ge \Pr{\bigcup_{i=1}^n \left( \overline{M_{u_i}}(v)\cap \exists(vu_i) \right)}.
\]

Notice that $Q_{u_i}(v) \subseteq \overline{M_{u_i}}(v)$, $Q_{u_i}(v)$ and $\overline{M_{u_i}}(v) \backslash Q_{u_i}(v)$ partition the event $\overline{M_{u_i}}(v)$. Moreover, the event $\cap_{j \ne i} \nexists (vu_j)$ is disjoint with $\cup_{j \ne i}(\overline{M_{u_i}}(v)\cap \exists(vu_j))$. We have that
\begin{align*}
\Pr{M_v} \ge & \Pr{\bigcup_{i=1}^n \left( \overline{M_{u_i}}(v)\cap \exists(vu_i) \right)} \\
\ge & \Pr{\bigcup_{i=1}^n \left( \overline{Q_{u_i}}(v)\cap \exists(vu_i) \right)} + \sum_{i=1}^{n} \Pr{\overline{M_{u_i}}(v) \backslash Q_{u_i}(v) \cap \exists(vu_i) \cap_{j \ne i} \nexists(vu_j)}.
\end{align*}
\end{proof}

\begin{lemma}
	\label{lem:rone}
\begin{equation}
\Pr{\bigcup_{i=1}^n \left( Q_{u_i}(v)\cap \exists(vu_i) \right)} \ge \sum_{i=1}^{n} x_{vu_i} \cdot \left( 1- \left(1-q_{u_i}(v) \cdot y_{vu_i} \right)^{\frac{1}{x_{vu_i}}} \right).
\end{equation}
\end{lemma}
\begin{proof}
Notice that 1) the event $Q_{u_i}(v) \cap \exists(vu_i)$ only the depends on the random realizations of edges incident to $u_i$; 2) the edges incident to $u_i$ are disjoint with the edges incident to $u_j$ for any $i\ne j$. That is, the events $Q_{u_i}(v) \exists (vu_i)$ are independent. Hence,
\begin{align*}
\Pr{\bigcup_{i=1}^n \left( Q_{u_i}(v)\cap \exists(vu_i) \right)} = & 1 - \prod_{i=1}^{n} \left( 1 - \Pr{Q_{u_i}(v) \cap \exists(vu_i)} \right)\\
= & 1 - \prod_{i=1}^{n} (1-q_{u_i}(v) \cdot y_{vu_i}) = 1 - \exp\left(\sum_{i=1}^{n} \ln(1-q_{u_i}(v) \cdot y_{vu_i}) \right) \\
= & 1 - \exp\left( \sum_{i=1}^{n} x_{vu_i} \cdot \frac{\ln(1-q_{u_i}(v) \cdot y_{vu_i})}{x_{vu_i}} + \left( 1-\sum_{i}x_{vu_i} \right) \cdot 0 \right) \\
\ge & \sum_{i=1}^{n} x_{vu_i} \cdot \left( 1-(1-q_{u_i}(v) \cdot y_{vu_i})^{1/x_{vu_i}} \right) \tag{by Jesnsen's inequality}
\end{align*}
where we use the concavity of $1-\exp(-z)$ in the inequality.
\end{proof}

\begin{lemma}
	\label{lem:rtwo}
\begin{equation}
\Pr{\overline{M_{u_i}}(v) \backslash Q_{u_i}(v) \cap \exists(vu_i) \cap_{j \ne i} \nexists(vu_j)} \ge e^{-c} \cdot \frac{y_{vu_i}}{1-y_{vu_i}} \cdot \left( \Pr{\overline{M_{u_i}}(v)} - \Pr{Q_{u_i}(v)}  \right).
\end{equation}
\end{lemma}
\begin{proof}
\begin{align*}
& \Pr{\overline{M_{u_i}}(v) \backslash Q_{u_i}(v) \cap \exists(vu_i) \cap_{j \ne i} \nexists(vu_j)} \\
= & \Pr{\exists(vu_i) \cap_{j \ne i} \nexists(vu_j)} \cdot \Pr{\overline{M_{u_i}}(v) \backslash Q_{u_i}(v) \Big| \exists(vu_i) \cap_{j \ne i} \nexists(vu_j) } \\
= & \Pr{\exists(vu_i) \cap_{j \ne i} \nexists(vu_j)} \cdot \left( \Pr{\overline{M_{u_i}}(v) \Big| \exists(vu_i) \cap_{j \ne i} \nexists(vu_j)} - \Pr{ Q_{u_i}(v) \Big| \exists(vu_i) \cap_{j \ne i} \nexists(vu_j)} \right) \\
= & \Pr{\exists(vu_i) \cap_{j \ne i} \nexists(vu_j)} \cdot \left( \Pr{\overline{M_{u_i}}(v) \Big| Q_{v}(u_i)} - \Pr{ Q_{u_i}(v)} \right) \tag{$*$} \\
\ge & \Pr{\exists(vu_i) \cap_{j \ne i} \nexists(vu_j)} \cdot \left( \Pr{\overline{M_{u_i}}(v)} - \Pr{Q_{u_i}(v)}  \right) \tag{by Lemma~\ref{lem:conditional_unmatch}} \\
= & y_{uv_i} \cdot \prod_{j\ne i}(1-y_{vu_j}) \cdot \left( \Pr{\overline{M_{u_i}}(v)} - \Pr{Q_{u_i}(v)}  \right) \\
\ge & e^{-c} \cdot \frac{y_{vu_i}}{1-y_{vu_i}} \cdot \left( \Pr{\overline{M_{u_i}}(v)} - \Pr{Q_{u_i}(v)}  \right).
\end{align*}
In equation $(*)$, we use that $\overline{M_{u_i}}(v)$ is independent of the edges that arrive after $(vu_i)$.
In the last inequality, we use that $\prod_{j} (1-y_{vu_j}) = \prod_{e\in E_v} (1-y_e) \approx \exp(-\sum_{e}y_e) \ge e^{-c}$.
\end{proof}

\begin{lemma}
	\label{lem:conditional_unmatch}
	For any vertices $v \in L, u \in R$, $\Pr{\overline{M_u}(v) | Q_{v}(u)} \ge \Pr{\overline{M_u}(v)}$.
\end{lemma}
\zhihao{to prove. Move to earlier places. This would be useful somewhere else.}

For any pair of vertices $v \in L, u \in R$, define 
\begin{align*}
& \rone(vu) \eqdef x_{vu} \cdot (1 - (1-q_u(v) \cdot y_{vu})^{1/x_{vu}}); \\
\text{and } & \rtwo(vu) \eqdef \frac{y_{vu}}{1-y_{vu}} \cdot \left( \Pr{\overline{M_{u}}(v)} - \Pr{Q_{u}(v)}  \right).
\end{align*}

To sum up, by Lemmas~\ref{lem:prob_v_match}, \ref{lem:rone} and \ref{lem:rtwo}, we have that
\[
\Pr{M_v} \ge \sum_{u} \left( \rone(vu) + e^{-c} \cdot \rtwo(vu) \right).
\] 
Summing over $v \in L$, we have that
\[
\greedy = \sum_{v \in L} \Pr{M_v} \ge \sum_{v \in L} \sum_{u \in R} \left( \rone(vu) + e^{-c} \cdot \rtwo(vu) \right).
\]
In other words, these two quantities capture the contribution of edge $(vu)$ to the performance of greedy (using our analysis).
Finally, we prove the following subdivision lemma.
\begin{lemma}
\begin{equation}
	\rone(vu) + e^{-c} \cdot \rtwo(vu) \ge \sum_{e \in E_{vu}} \left( \rone(e) + e^{-c-ce^{-c}} \cdot \rtwo(e) \right).
\end{equation}
\end{lemma}

\begin{proof}
Suppose there are $k$ parallel edges $\{e_1,\cdots,e_k\}$ in $E_{vu}$. We have that $\sum_{j} x_{e_j} = x_{vu}$ and $\prod_{j} (1-y_{e_j}) = (1-y_{vu})$.
We first consider the difference between the $\rone$ terms.
\begin{align}
\rone(vu) - \sum_{j} \rone(e_j) = & \sum_{j} x_{e_j} \cdot \exp \left( - \frac{q_u(e_j)\cdot y_{e_j}}{x_{e_j}} \right)  - x_{vu} \cdot \left( 1-q_{u}(v) \cdot y_{vu} \right)^{\frac{1}{x_{vu}}} \notag \\
\ge & x_{vu} \cdot \left( \exp\left( - \frac{\sum_{j}q_{u}(e_j)\cdot y_{e_j}}{x_{vu}} \right) - \left( 1-q_{u}(v) \cdot y_{vu} \right)^{\frac{1}{x_{vu}}} \right) \tag{by Jenson's inequality}\\
= & x_{vu} \cdot \left( \exp\left( - \frac{q_u(v) \cdot y_{vu}}{x_{vu}} \right) - \left( 1-q_{u}(v) \cdot y_{vu} \right)^{\frac{1}{x_{vu}}} \right). \label{eq:rone_increment}
%\ge & (1-q_{u}(v) \cdot y_{vu})^{1/x_{vu} - 1} \left( \exp(-q_{u}(v)\cdot y_{vu}) - 1 + q_{u}(v) \cdot y_{vu} \right).
\end{align}
Next we consider the difference between the $\rtwo$ terms.
Note that the probability $u$ is unmatched decreases as time proceeds. We have that $\Pr{\overline{M_{u}}(v)} \ge \Pr{\overline{M_{u}}(e_j)}$ for all $j$. Next,
\[
\frac{y_{vu}}{1-y_{vu}} = \frac{1-\prod_{j}(1-y_{e_j})}{\prod_{j}(1-y_{e_j})} \ge \sum_{j} y_{e_j}.
\]
Thus,
\begin{align}
\sum_{j}\rtwo(e_j) - \rtwo(vu) = & \sum_{j} y_{e_j} \cdot \left( \Pr{\overline{M_{u}}(e_j)} - \Pr{Q_{u}(e_j)} \right) - \frac{y_{vu}}{1-y_{vu}} \cdot \left( \Pr{\overline{M_{u}}(v)} - \Pr{Q_{u}(v)} \right) \notag\\
\le & \sum_{j} y_{e_j} \cdot \left( \Pr{\overline{M_{u}}(v)} - \Pr{Q_{u}(e_j)} \right) - \sum_{j} y_{e_j} \cdot \left( \Pr{\overline{M_{u}}(v)} - \Pr{Q_{u}(v)} \right) \notag \\
= & \sum_{j} y_{e_j} \cdot \left(\Pr{Q_u(v)} - \Pr{Q_u(e_j)} \right) \notag \\
= & \sum_{j} y_{e_j} \cdot (1 - \prod_{i<j} (1-y_{e_i}))\cdot q_u(v) \notag \\
\approx & \sum_{j} y_{e_j} \cdot (1 - e^{-\sum_{i<j} y_{e_i}}) \cdot q_u(v) \notag \\
\approx & \int_{0}^{\sum_{j} y_{e_j}} (1 - e^{-y}) \dd y \cdot q_u(v) \notag \\
= & \left( \sum_{j} y_{e_j} + e^{-\sum_{j} y_{e_j}} - 1 \right) \cdot q_u(v) = ( -\ln(1-y_{vu}) - y_{vu} ) \cdot q_u(v). \label{eq:rtwo_decrement}
\end{align}
For notation simplicity, in the rest of the proof, we use $x,y,q$ to denote $x_{vu},y_{vu},q_u(v)$ respectively.
We have the fact that $y \le 1-e^{-cx}$ and $\frac{e^{-c}}{1-y} \le q \le 1$.

By Equation~\eqref{eq:rone_increment} and \eqref{eq:rtwo_decrement}, it suffices to prove that
\[
h(x,y,q) \eqdef \frac{x \cdot \left( e^{-\frac{qy}{x}} - (1-qy)^{\frac{1}{x}} \right)}{(-\ln(1-y)-y) q} \ge e^{-c} \cdot e^{-c e^{-c}}.
\]
\begin{claim}
	We have the following mathematical facts:
\begin{enumerate}
	\item For any $1>a>b>0$, $f(x)= x\cdot (a^{1/x} - b^{1/x})$ is an increasing function of $x$.
	\item For any $d>1$, $g(z) = \frac{e^{-dz} - (1-z)^d}{z}$ increases first and then decreases.
\end{enumerate}	
\end{claim}
\zhihao{to prove}

Fix $y,q$, the first statement tells that the minimum of $h(x,y,q)$ is achieved when $y=1-e^{-cx}$.
Moreover, fix $x,y$, we rewrite $h$ as the following.
\[
h(x,y,q) = \frac{xy}{-\ln(1-y)-y} \cdot \frac{\left( e^{-\frac{qy}{x}} - (1-qy)^{\frac{1}{x}} \right)}{qy}
\]
By the second statement, the minimum must be achieved when $q=1$ or $\frac{e^{-c}}{1-y}$. We consider the two cases separately.

\zhihao{to prove}
\begin{enumerate}
\item When $y=1-e^{-cx}, q=1$, the minimum is achieved when $x \to 0$, 
\[
\lim_{x\to 0} h(x,1-e^{-cx},1) = e^{-c}.
\]
\item When $y = 1-e^{-cx}, q=\frac{e^{-c}}{1-y}=e^{cx-c}$, the minimum is achieved when $x \to 0$,
\[
\lim_{x \to 0} h(x,1-e^{-cx},e^{cx-c}) = e^{-c} \cdot e^{-c\cdot e^{-c}}.
\]
\end{enumerate}
\end{proof}


==> prune_greedy.tex <==
Consider the following algorithm.
\begin{enumerate}
	\item Solve the LP.
	\item Prune the graph by decreasing the probabilities of each edge from $p_e$ to $y_e = \min (p_e, c x_e)$, where $c>1$ is a constant to be optimized.
	\item Run Greedy.
\end{enumerate}

Define the events $Q_e$ to be the same as in the regular case.
\begin{definition}
Let $u\in L, v\in R$. For each edge $e \in E_{uv}$, define $Q_e$ to be the event that $e$ exists and is the first realized edge of $E_u$ in the given arrival order. Let $q_e = \Pr{Q_e}$.
\end{definition}

Lemma 2 in the original version still holds.
\begin{lemma}
	The expected size of matching is at least 
	$
	\sum\limits_{u \in L} \sum\limits_{e \in E_u} x_e \cdot \left(1 - e^{-\frac{q_e}{x_e}}\right).
	$
\end{lemma}

But we now have a different mathematical program to solve.

\begin{align*}
\min_{(p_i\le 1), (x_i\ge 0)} &  \sum_{i=1}^k x_i\cdot \left( 1-e^{-\frac{q_i}{x_i}} \right) / \sum\limits_{i=1}^{k} x_i \\
\text{s.t. } & q_i = \prod_{j<i} (1-y_j) \cdot y_i, ~~\forall i \in [k] \\
& \sum\limits_{i \in S} x_i \leq 1 - \prod\limits_{i \in S} (1 - p_i),~~~\quad\quad\quad, \forall S \subseteq [k]
\end{align*}

The analysis of this mathematical program goes similarly as the old one. Following the original steps, we prove the statements:
\begin{enumerate}
	\item W.l.o.g. all $x_i$'s are the same.
	\item $y_i$'s are decreasing. Then $\vec{y} = (cx, \cdots, cx, p_{l+1}, \cdots, p_k)$.
	\item The constraints are tight for the suffices of $\vec{p}$. Then $p_i = \frac{x}{1-(k-i)x}$ for $i > l$. 
\end{enumerate}
If the above steps still go through, 
\begin{align*}
q_i = \begin{cases}
(1-cx)^{i-1} \cdot cx & i \le l \\
(1-cx)^l \cdot \frac{1-(k-l)x}{1-(k-i+1)x} \cdot \frac{x}{1-(k-i)x} & i > l
\end{cases}
\end{align*}
The worst case would be $kx=1$ and $p_{l+1} = cx$, i.e. $lx \approx \frac{1}{c}$. The ratio is then
\[
\int_0^{\frac{1}{c}} 1-e^{-ce^{-ct}}dt + \int_{\frac{1}{c}}^{1} 1-e^{-\frac{1}{cet^2}} dt \ge 0.503,
\]
when $c=1.7$.
